Human Evaluation and Correlation with Automatic Metrics in Consultation Note Generation

In recent years, machine learning models have rapidly become better at generating clinical consultation notes; yet, there is little work on how to properly evaluate the generated consultation notes to understand the impact they may have on both the clinician using them and the patient's clinical safety. To address this we present an extensive human evaluation study of consultation notes where 5 clinicians (i) listen to 57 mock consultations, (ii) write their own notes, (iii) post-edit a number of automatically generated notes, and (iv) extract all the errors, both quantitative and qualitative. We then carry out a correlation study with 18 automatic quality metrics and the human judgements. We find that a simple, character-based Levenshtein distance metric performs on par if not better than common model-based metrics like BertScore. All our findings and annotations are open-sourced.

==> sections/literature_review_longtable.tex <==



% \begin{center}
% \small
% \begin{longtable}{>{\raggedright}p{1.3cm}|p{5.5cm}|>{\raggedright}p{2cm}|>{\raggedright}p{5.5cm}}
% \caption{Summary of studies and evaluations on Note Generation up to date. We place question marks for values that we couldn't find in the paper.} \label{tab:notegen-studies} \\


% \hline \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation} \\ \hline 
% \endfirsthead


% \multicolumn{4}{c}%
% {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
% \hline \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation} \\ \hline 
% \endhead

% \hline \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
% \endfoot

% \hline \hline
% \endlastfoot

%         \citet{moen2016evaluation} & Evaluation of automatically generated clinical discharge summarises to find out if there is a correlation between the automatic evaluation and the manual evaluation. The manual evaluation is performed by domain experts. & Rouge (1, 2, L, SU4) & 
%         \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 3 domain experts \newline
% \textbf{Dataset}: 40 notes \newline
% \textbf{Criteria}: 30 items (Long-term diagnoses, Reason for admission, Assessment of the future, etc.)  \newline
% \textbf{Tasks}: likert scale (not relevant, not included, partially included and fully included) \newline
% \textbf{Correlation}: automatic metrics agreed with human evaluation \newline
% \textbf{Insights}: subjects found the 30 item scale too difficult and detailed to assess. \hline


%         \cite{moen2016comparison} & Follow up to \cite{moen2016evaluation}. A suite of extractive text summarisation methods for summarising the free text content of care episodes. & Rouge (1, 2, L, SU4) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 3 domain experts \newline
% \textbf{Dataset}: 160 notes \newline
% \textbf{Criteria}: 10 items (subset of previous study) \newline
% \textbf{Task}: binary (present, absent) \newline
% \textbf{Agreement}: intraclass correlation coefficient \citep{shrout1979intraclass} = 0.744 \hline
        
        
%         \citet{alsentzer2018extractive} & Extractive summarisation of EHR discharge notes and an LSTM model to sequentially label topics of history of present illness notes. & Ontology-based fact extractor, computing precision, recall and f-score & -- \hline
        
%         \citet{finley2018automated} & Implementation of an automated medical scribe to be used either as a scalable, standardized, and economical alternative to human scribes or as an assistive tool for them, providing a first draft of a report along with a convenient means to modify it. & -- & -- \hline
        
%         \citet{zhang2018learning} & Generation of radiology impressions with neural sequence-to-sequence learning, and a customized neural model for this task, which learns to encode the study background information and use this information to guide the decoding process. & Rouge (1, 2, L) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 1 domain expert \newline
% \textbf{Dataset}: 100 notes \newline
% \textbf{Criteria}: 1 \newline 
% \textbf{Task}: binary (choose the ``best'' note between the generated and reference)\hline
        
%         \citet{kazi2019automatically} & Generation of psychiatric case notes from digital transcripts by (1) predicting semantic topics for segments of transcripts using supervised machine learning, and (2) generating formal text of those segments using natural language processing. & -- & --\hline

%         \citet{liu2019topic} & Pointer-networks for summarising nurse-to-patient dialogues. & Rouge (1, 2, L), training loss & --\\ \hline
        
%         \citet{macavaney2019ontology} & A sequence-to-sequence abstractive summarization model augmented with domain-specific ontological information to enhance content selection and summary generation of radiology reports. & Rouge (1, 2, and L) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 1 domain expert \newline
% \textbf{Dataset}: 100 notes \newline
% \textbf{Task}: likert scale (1 to 5) \newline
% \textbf{Criteria}: \newline
% - Readability. Impression is understandable (5) or gibberish (1) \newline
% - Accuracy. Impression is fully accurate (5), or contains critical errors (1) \newline
% - Completeness. Impression contains all important information (5), or is missing important points (1). \hline
        
%         \citet{zhang2020optimizing} & Evaluate the factual correctness of a generated summary by fact-checking it automatically against its reference using an information extraction module. Propose a training strategy which optimizes a neural summarization model with a factual correctness reward via reinforcement learning. Apply the proposed method to the summarization of radiology reports, where factual correctness is a key requirement. & Rouge (1, 2, and L). Ontology based fact-extractor (F-score). & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 2 domain experts \newline
% \textbf{Dataset}: 50 consultations (3 notes each: two generated, one human reference) \newline
% \textbf{Criteria}: 
% (1) fluency, \newline
% (2) factual correctness and completeness, \newline
% (3) overall quality \newline
% \textbf{Task}: rank the 3 notes for each criteria (ties allowed)\hline
        
        
%         \citet{enarvi2020generating} & Automatic creation of medical reports from ASR-generated patient-doctor conversational transcripts using an end-to-end neural summarization approach. They explore both recurrent neural network (RNN) and Transformer-based sequence-to-sequence architectures for summarizing medical conversations. They provide enhancements to these architectures, such as the pointer-generator network that facilitates copying parts of the conversations to the reports, and a hierarchical RNN encoder that makes RNN training three times faster with long inputs. & Rouge-L, ML fact-extractor (proprietary) & --\hline

%         \citet{joshi2020dr} & Their approach is a variation of the pointer generator network where they introduce a penalty on the generator distribution, and they explicitly model negations. The model also captures important properties of medical conversations such as medical knowledge coming from standardized medical ontologies better than when those concepts are introduced explicitly. & Rouge, Medical Concept Coverage (F-score with UMLS), Negex \citep{harkema2009context} for negated symptoms.  & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 2 domain experts \newline
% \textbf{Criteria / Task}: \newline
% - percentage of medical concepts covered in the note (recall), by selecting All (100\%), Most (at least 75\%), Some (at least 1 fact but less than 75\%), None (0\%) labels \newline
% - rank two generated notes according to which one ``is better'' \newline
% \textbf{Dataset}: 167 consultations \newline
% \textbf{Agreement}: ?\hline
        
%         \citet{krishna-etal-2021-generating} & Generate SOAP notes from doctor-patient conversation via: (i) extracting important utterances relevant to each summary section; (ii) clustering together related utterances; and then (iii) generating one summary sentence per cluster. & Rouge (1, 2, L) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: ? ``trained human annotators'', who also drafted the dataset \newline
% \textbf{Dataset}: 45 consultations \newline
% \textbf{Criteria}:  factually correct, incoherent, irrelevant, redundant, or
% placed under an inappropriate section, comprehensiveness and extent of verbatim copying from conversation \newline
% \textbf{Task}: 5-point likert scale \newline
% \textbf{Agreement}: ?\hline
        
%         \citet{maas2020care2report} & Automate the process of medical reporting through the integration of speech and action recognition technology with semantic interpretation based on knowledge graphs. This paper presents a dialogue summarization pipeline that transforms speech into a medical report via transcription and formal representation. & Planned for future work, using BLEU. & Planned for future work. \newline
% \textbf{Criteria}: correctness, completeness, and fluency of the generated reports\\ \hline
        
%         \citet{molenaar2020medical} & A note generation pipeline for consultations on ear infections based on 4 components: speech to Text (Google), triple extraction (e.g. Ear, hasSymptom, Pain), triple matching (against ontology) and categorisation, report generation (triples to text with NaturalOWL). & -- & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: ? \newline
% \textbf{Dataset}: 8 consultations \newline
% \textbf{Criteria}: Extract ``items'' (akin to noun chunks) and compare to reference note \newline
% \textbf{Task}: compute precision, recall, f-score, and false positives. \newline
% \textbf{Agreement}: ? \hline
        
%         \citet{chintagunta2021medically} & They scale 210 human labeled examples (consultation transcripts and notes) to yield results comparable to using 6400 human labeled examples (~30x) leveraging low-shot learning and an ensemble method. Then, they train an end-to-end abstractive summariser. & Rouge, Medical Concept Coverage (F-score with UMLS), Negex \citep{harkema2009context} for negated syntoms & \textbf{Type}: intrinsic\newline
% \textbf{Subjects}: ?\newline
% \textbf{Criteria / Task}: \newline
% - percentage of medical concepts covered in the note (recall), by selecting All (100\%), Most (at least 75\%), Some (at least
% 1 fact but less than 75\%), None (0\%) labels\newline
% - rank two generated notes according to which one ``is best according to a usability perspective. Usability was defined as whether the summary
% could stand in as a replacement for reading the dialogue snippet" \newline
% \textbf{Dataset}: ? \newline
% \textbf{Agreement}: ?\hline
        
%         \citet{yim2021towards} & They describe a corpus creation method and baseline systems for two NLP tasks, clinical dialogue2note sentence alignment and clinical dialogue2note snippet summarization. & Bleu, Rouge (1, 2, L) & \textbf{Type}: intrinsic\newline
% \textbf{Dataset}: 10 samples for each of 6 snippet sections in the note\newline
% \textbf{Subjects}: 1 annotator with medical degree\newline
% \textbf{Criteria / Task}:\newline
% - rank the four generated notes based on ?\newline
% - relevancy, factual accuracy, writing-style, completeness, and overall with a 5-point likert scale\hline
        
%         \citet{moramarco2021preliminary} & They propose a semi-automatic approach whereby physicians post-edit generated notes before submitting them.
% They conduct a preliminary study on the time
% saving of automatically generated consultation
% notes with post-editing. Their evaluators are
% asked to listen to mock consultations and to
% post-edit three generated notes. & -- & \textbf{Type}: intrinsic\newline
% \textbf{Dataset}: 3 consultations, 3 notes each\newline
% \textbf{Subjects}: 3 consulting clinicians\newline
% \textbf{Criteria / Task}:\newline
% - time to post-edit the note\newline
% - count of incorrect statements, major omissions, minor omissions\newline
% - coherence likert scale \hline

%         \citet{zhang2021leveraging} & They explore the feasibility of using pretrained transformer models for automatically summarizing doctor patient conversations directly from transcripts. They evaluate multiple methods for handling long conversations, comparing them to the obvious baseline of truncating the conversation to fit the pretrained model length limit. They introduce a multistage approach that tackles the task by learning two finetuned models. They conduct both an automatic evaluation (through ROUGE and two concept-based metrics focusing on medical findings) and a human evaluation (through qualitative examples from literature, assessing hallucination, generalization, fluency, and general quality of the generated summaries). & Rouge, IE based metric & \textbf{Type}: intrinsic\newline
% \textbf{Dataset}: 10 conversation, 5 notes each\newline
% \textbf{Subjects}: 2 ``domain experts''\newline
% \textbf{Criteria / Task}:\newline
% - fluency: How fluent is the text generated?\newline
% - relevancy: Are contents relevant for HPI?\newline
% - missing: Are any key findings missing?\newline
% - hallucination: Are any findings hallucinated
% or inaccurate?\newline
% - repetition: Are there repetitive sentences?\newline
% - contradiction: Are any sentences contradicting each other?

% \end{longtable}
% \end{center}

==> sections/literature_review_table.tex <==
% \begin{table*}[t]
%     \centering
%     \begin{tabular}{p{1.6cm}|p{5.4cm}|p{2cm}|p{5.4cm}}
%     \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation}\\\hline
%         \citet{moen2016evaluation} & Evaluation of automatically generated clinical discharge summarises to find out if there is a correlation between the automatic evaluation and the manual evaluation. The manual evaluation is performed by domain experts. & Rouge (1, 2, L, SU4) & 
%         \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 3 domain experts \newline
% \textbf{Dataset}: 40 notes \newline
% \textbf{Criteria}: 30 items (Long-term diagnoses, Reason for admission, Assessment of the future, etc.)  \newline
% \textbf{Tasks}: likert scale (not relevant, not included, partially included and fully included) \newline
% \textbf{Correlation}: automatic metrics agreed with human evaluation \newline
% \textbf{Insights}: subjects found the 30 item scale too difficult and detailed to assess. \\\hline


%         \cite{moen2016comparison} & Follow up to \cite{moen2016evaluation}. A suite of extractive text summarisation methods for summarising the free text content of care episodes. & Rouge (1, 2, L, SU4) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 3 domain experts \newline
% \textbf{Dataset}: 160 notes \newline
% \textbf{Criteria}: 10 items (subset of previous study) \newline
% \textbf{Task}: binary (present, absent) \newline
% \textbf{Agreement}: intraclass correlation coefficient \citep{shrout1979intraclass} = 0.744 \\\hline
        
   
%         \citet{alsentzer2018extractive} & Extractive summarisation of EHR discharge notes and an LSTM model to sequentially label topics of history of present illness notes. & Ontology-based fact extractor, computing precision, recall and f-score & -- \\\hline
        
%         \citet{finley2018automated} & Implementation of an automated medical scribe to be used either as a scalable, standardized, and economical alternative to human scribes or as an assistive tool for them, providing a first draft of a report along with a convenient means to modify it. & -- & -- \\\hline
        
%         \citet{zhang2018learning} & Generation of radiology impressions with neural sequence-to-sequence learning, and a customized neural model for this task, which learns to encode the study background information and use this information to guide the decoding process. & Rouge (1, 2, L) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 1 domain expert \newline
% \textbf{Dataset}: 100 notes \newline
% \textbf{Criteria}: 1 \newline 
% \textbf{Task}: binary (choose the ``best'' note between the generated and reference)\\\hline
%         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             \end{tabular}
%     \caption{Summary of studies and evaluations on Note Generation up to date. We place question marks for values that we couldn't find in the paper.} 
%     \label{tab:notegen-studies}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{p{1.6cm}|p{5.4cm}|p{2cm}|p{5.4cm}}
%     \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation}\\\hline
%       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
%         \citet{kazi2019automatically} & Generation of psychiatric case notes from digital transcripts by (1) predicting semantic topics for segments of transcripts using supervised machine learning, and (2) generating formal text of those segments using natural language processing. & -- & --\\\hline

%         \citet{liu2019topic} & Pointer-networks for summarising nurse-to-patient dialogues. & Rouge (1, 2, L), training loss & --\\ \\\hline
        
%         \citet{macavaney2019ontology} & A sequence-to-sequence abstractive summarization model augmented with domain-specific ontological information to enhance content selection and summary generation of radiology reports. & Rouge (1, 2, and L) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 1 domain expert \newline
% \textbf{Dataset}: 100 notes \newline
% \textbf{Task}: likert scale (1 to 5) \newline
% \textbf{Criteria}: \newline
% - Readability. Impression is understandable (5) or gibberish (1) \newline
% - Accuracy. Impression is fully accurate (5), or contains critical errors (1) \newline
% - Completeness. Impression contains all important information (5), or is missing important points (1). \\\hline
        
%         \citet{zhang2020optimizing} & Evaluate the factual correctness of a generated summary by fact-checking it automatically against its reference using an information extraction module. Propose a training strategy which optimizes a neural summarization model with a factual correctness reward via reinforcement learning. Apply the proposed method to the summarization of radiology reports, where factual correctness is a key requirement. & Rouge (1, 2, and L). Ontology based fact-extractor (F-score). & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 2 domain experts \newline
% \textbf{Dataset}: 50 consultations (3 notes each: two generated, one human reference) \newline
% \textbf{Criteria}: 
% (1) fluency, \newline
% (2) factual correctness and completeness, \newline
% (3) overall quality \newline
% \textbf{Task}: rank the 3 notes for each criteria (ties allowed)\\\hline
        
%         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             \end{tabular}
%     \caption{Continuation: Summary of studies and evaluations on Note Generation up to date. We place question marks for values that we couldn't find in the paper.} 
%     \label{tab:notegen-studies-2}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{p{1.6cm}|p{5.4cm}|p{2cm}|p{5.4cm}}
%     \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation}\\\hline
%       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%          
%         \citet{enarvi2020generating} & Automatic creation of medical reports from ASR-generated patient-doctor conversational transcripts using an end-to-end neural summarization approach. They explore both recurrent neural network (RNN) and Transformer-based sequence-to-sequence architectures for summarizing medical conversations. They provide enhancements to these architectures, such as the pointer-generator network that facilitates copying parts of the conversations to the reports, and a hierarchical RNN encoder that makes RNN training three times faster with long inputs. & Rouge-L, ML fact-extractor (proprietary) & --\\\hline
 
%         \citet{joshi2020dr} & Their approach is a variation of the pointer generator network where they introduce a penalty on the generator distribution, and they explicitly model negations. The model also captures important properties of medical conversations such as medical knowledge coming from standardized medical ontologies better than when those concepts are introduced explicitly. & Rouge, Medical Concept Coverage (F-score with UMLS), Negex \citep{harkema2009context} for negated symptoms.  & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: 2 domain experts \newline
% \textbf{Criteria / Task}: \newline
% - percentage of medical concepts covered in the note (recall), by selecting All (100\%), Most (at least 75\%), Some (at least 1 fact but less than 75\%), None (0\%) labels \newline
% - rank two generated notes according to which one ``is better'' \newline
% \textbf{Dataset}: 167 consultations \newline
% \textbf{Agreement}: ?\\\hline


       
%         \citet{krishna-etal-2021-generating} & Generate SOAP notes from doctor-patient conversation via: (i) extracting important utterances relevant to each summary section; (ii) clustering together related utterances; and then (iii) generating one summary sentence per cluster. & Rouge (1, 2, L) & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: ? ``trained human annotators'', who also drafted the dataset \newline
% \textbf{Dataset}: 45 consultations \newline
% \textbf{Criteria}:  factually correct, incoherent, irrelevant, redundant, or
% placed under an inappropriate section, comprehensiveness and extent of verbatim copying from conversation \newline
% \textbf{Task}: 5-point likert scale \newline
% \textbf{Agreement}: ?\\\hline
%               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             \end{tabular}
%     \caption{Continuation: Summary of studies and evaluations on Note Generation up to date. We place question marks for values that we couldn't find in the paper.} 
%     \label{tab:notegen-studies-3}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{p{1.6cm}|p{5.4cm}|p{2cm}|p{5.4cm}}
%     \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation}\\\hline
%       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%        
%         \citet{maas2020care2report} & Automate the process of medical reporting through the integration of speech and action recognition technology with semantic interpretation based on knowledge graphs. This paper presents a dialogue summarization pipeline that transforms speech into a medical report via transcription and formal representation. & Planned for future work, using BLEU. & Planned for future work. \newline
% \textbf{Criteria}: correctness, completeness, and fluency of the generated reports\\ \hline
   
%         \citet{molenaar2020medical} & A note generation pipeline for consultations on ear infections based on 4 components: speech to Text (Google), triple extraction (e.g. Ear, hasSymptom, Pain), triple matching (against ontology) and categorisation, report generation (triples to text with NaturalOWL). & -- & \textbf{Type}: intrinsic \newline
% \textbf{Subjects}: ? \newline
% \textbf{Dataset}: 8 consultations \newline
% \textbf{Criteria}: Extract ``items'' (akin to noun chunks) and compare to reference note \newline
% \textbf{Task}: compute precision, recall, f-score, and false positives. \newline
% \textbf{Agreement}: ? \\\hline
        
%         \citet{chintagunta2021medically} & They scale 210 human labeled examples (consultation transcripts and notes) to yield results comparable to using 6400 human labeled examples (~30x) leveraging low-shot learning and an ensemble method. Then, they train an end-to-end abstractive summariser. & Rouge, Medical Concept Coverage (F-score with UMLS), Negex \citep{harkema2009context} for negated syntoms & \textbf{Type}: intrinsic\newline
% \textbf{Subjects}: ?\newline
% \textbf{Criteria / Task}: \newline
% - percentage of medical concepts covered in the note (recall), by selecting All (100\%), Most (at least 75\%), Some (at least
% 1 fact but less than 75\%), None (0\%) labels\newline
% - rank two generated notes according to which one ``is best according to a usability perspective. Usability was defined as whether the summary
% could stand in as a replacement for reading the dialogue snippet" \newline
% \textbf{Dataset}: ? \newline
% \textbf{Agreement}: ?\\\hline
        
%         \citet{yim2021towards} & They describe a corpus creation method and baseline systems for two NLP tasks, clinical dialogue2note sentence alignment and clinical dialogue2note snippet summarization. & Bleu, Rouge (1, 2, L) & \textbf{Type}: intrinsic\newline
% \textbf{Dataset}: 10 samples for each of 6 snippet sections in the note\newline
% \textbf{Subjects}: 1 annotator with medical degree\newline
% \textbf{Criteria / Task}:\newline
% - rank the four generated notes based on ?\newline
% - relevancy, factual accuracy, writing-style, completeness, and overall with a 5-point likert scale\\\hline
%         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             \end{tabular}
%     \caption{Continuation: Summary of studies and evaluations on Note Generation up to date. We place question marks for values that we couldn't find in the paper.} 
%     \label{tab:notegen-studie-4}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{p{1.6cm}|p{5.4cm}|p{2cm}|p{5.4cm}}
%     \textbf{Paper} & \textbf{Approach} & \textbf{Automatic Evaluation} & \textbf{Human Evaluation}\\\hline
%       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%          
%         \citet{moramarco2021preliminary} & They propose a semi-automatic approach whereby physicians post-edit generated notes before submitting them.
% They conduct a preliminary study on the time
% saving of automatically generated consultation
% notes with post-editing. Their evaluators are
% asked to listen to mock consultations and to
% post-edit three generated notes. & -- & \textbf{Type}: intrinsic\newline
% \textbf{Dataset}: 3 consultations, 3 notes each\newline
% \textbf{Subjects}: 3 consulting clinicians\newline
% \textbf{Criteria / Task}:\newline
% - time to post-edit the note\newline
% - count of incorrect statements, major omissions, minor omissions\newline
% - coherence likert scale \\\hline

%         \citet{zhang2021leveraging} & They explore the feasibility of using pretrained transformer models for automatically summarizing doctor patient conversations directly from transcripts. They evaluate multiple methods for handling long conversations, comparing them to the obvious baseline of truncating the conversation to fit the pretrained model length limit. They introduce a multistage approach that tackles the task by learning two finetuned models. They conduct both an automatic evaluation (through ROUGE and two concept-based metrics focusing on medical findings) and a human evaluation (through qualitative examples from literature, assessing hallucination, generalization, fluency, and general quality of the generated summaries). & Rouge, IE based metric & \textbf{Type}: intrinsic\newline
% \textbf{Dataset}: 10 conversation, 5 notes each\newline
% \textbf{Subjects}: 2 ``domain experts''\newline
% \textbf{Criteria / Task}:\newline
% - fluency: How fluent is the text generated?\newline
% - relevancy: Are contents relevant for HPI?\newline
% - missing: Are any key findings missing?\newline
% - hallucination: Are any findings hallucinated
% or inaccurate?\newline
% - repetition: Are there repetitive sentences?\newline
% - contradiction: Are any sentences contradicting each other?
%     \end{tabular}
%     \caption{Continuation: Summary of studies and evaluations on Note Generation up to date. We place question marks for values that we couldn't find in the paper.} 
%     \label{tab:notegen-studies-5}
% \end{table*}
